Self-calibrating Deep Photometric Stereo Networks

This paper proposes an uncalibrated photometric stereo method for non-Lambertian scenes based on deep learning. Unlike previous approaches that heavily rely on assumptions of specific reflectances and light source distributions, our method is able to determine both shape and light directions of a scene with unknown arbitrary reflectances observed under unknown varying light directions. To achieve this goal, we propose a two-stage deep learning architecture, called SDPS-Net, which can effectively take advantage of intermediate supervision, resulting in reduced learning difficulty compared to a single-stage model. Experiments on both synthetic and real datasets show that our proposed approach significantly outperforms previous uncalibrated photometric stereo methods.

==> figures/compare_quant_pf14.tex <==
    \makebox[0.065\textwidth]{\scriptsize } 
    \makebox[0.065\textwidth]{\scriptsize } 
    \makebox[0.081\textwidth]{\scriptsize Lambertian} 
    \makebox[0.081\textwidth]{\scriptsize Fabric} 
    \makebox[0.081\textwidth]{\scriptsize Plastic} 
    \makebox[0.081\textwidth]{\scriptsize Metallic-paint} 
    \\
    \includegraphics[width=0.065\textwidth]{images/Results/synth/lights_400_uniform}
    \includegraphics[width=0.065\textwidth]{images/Results/synth/lights_400_up}
    \includegraphics[width=0.081\textwidth]{images/Results/synth/samples/albedo_6_gm.jpg}
    \includegraphics[width=0.081\textwidth]{images/Results/synth/samples/white-fabric_gm.jpg}
    \includegraphics[width=0.081\textwidth]{images/Results/synth/samples/yellow-matte-plastic_gm.jpg}
    \includegraphics[width=0.081\textwidth]{images/Results/synth/samples/silver-metallic-paint2_gm.jpg}
    %\includegraphics[width=0.075\textwidth]{images/Results/synth/samples/specular-white-phenolic_gm.jpg}
    \\
    \makebox[0.13\textwidth]{\footnotesize (a) Light sources} 
    \makebox[0.324\textwidth]{\footnotesize (b) Examples for the five types of BRDFs} 

\begin{minipage}{0.1\textwidth}
    \centering
    \makebox[\textwidth]{\footnotesize  }
    \includegraphics[width=\textwidth]{images/Results/synth/lights_400_uniform}
    %\includegraphics[width=0.09\textwidth]{images/Results/synth/lights_400_narrow}
    %\includegraphics[width=0.09\textwidth]{images/Results/synth/lights_400_up}
    \\
    \vspace{-0.6em}
    \makebox[\textwidth]{\footnotesize  } 
    \includegraphics[width=\textwidth]{images/Results/synth/lights_400_up}
\end{minipage}
\begin{minipage}{0.30\textwidth}
    \centering
    \makebox[0.30\textwidth]{\scriptsize Lambertian} 
    \makebox[0.30\textwidth]{\scriptsize Fabric} 
    \\
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/albedo_6_gm.jpg}
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/white-fabric_gm.jpg}
    \\
    \vspace{-0.6em}
    \makebox[0.30\textwidth]{\scriptsize Plastic} 
    \makebox[0.30\textwidth]{\scriptsize Phenolic} 
    \makebox[0.30\textwidth]{\scriptsize Metallic-paint} 
    \\

    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/yellow-matte-plastic_gm.jpg}
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/specular-white-phenolic_gm.jpg}
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/silver-metallic-paint2_gm.jpg}
    \\
\end{minipage}
    \makebox[0.11\textwidth]{\footnotesize (a) Light sources} 
    \makebox[0.3\textwidth]{\footnotesize (b) Examples for the five types of BRDFs} 
\includegraphics[width=0.48\textwidth]{images/Results/synth/compare_PF14/dir_unif}\\
\vspace{-0.7em}
\makebox[0.4\textwidth]{\footnotesize (c) Light direction estimation results} \\
\includegraphics[width=0.48\textwidth]{images/Results/synth/compare_PF14/intens_unif}\\
\vspace{-0.7em}\makebox[0.4\textwidth]{\footnotesize (d) Light intensity estimation results} \\
\includegraphics[width=0.48\textwidth]{images/Results/synth/compare_PF14/normal_unif}\\
\vspace{-0.7em}\makebox[0.4\textwidth]{\footnotesize (e) Surface normal estimation results}
\\


==> figures/diffuse_merl.tex <==
\begin{minipage}{0.1\textwidth}
    \centering
    \makebox[\textwidth]{\footnotesize A}
    \includegraphics[width=\textwidth]{images/Results/synth/lights_400_uniform}
    %\includegraphics[width=0.09\textwidth]{images/Results/synth/lights_400_narrow}
    %\includegraphics[width=0.09\textwidth]{images/Results/synth/lights_400_up}
    \\
    \vspace{-0.6em}
    \makebox[\textwidth]{\footnotesize B} 
    \includegraphics[width=\textwidth]{images/Results/synth/lights_400_left}
\end{minipage}
\begin{minipage}{0.30\textwidth}
    \centering
    \makebox[0.32\textwidth]{\footnotesize diffuse} 
    \makebox[0.32\textwidth]{\footnotesize fabric} 
    \\
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/diffuse_240.jpg}
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/red-fabric_l_240_gm.jpg}
    \\
    \vspace{-0.6em}
    \makebox[0.32\textwidth]{\footnotesize plastic} 
    \makebox[0.32\textwidth]{\footnotesize phenolic} 
    \makebox[0.32\textwidth]{\footnotesize metallic-paint} 
    \\
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/red-plastic_l_240_gm.jpg}
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/red-phenolic_l_240_gm.jpg}
    \includegraphics[width=0.32\textwidth]{images/Results/synth/samples/red-metallic-paint_l_240_gm.jpg}
    \\
\end{minipage}
    \makebox[0.11\textwidth]{\footnotesize (a) Light source} 
    \makebox[0.3\textwidth]{\footnotesize (b) Examples for the five types of BRDFs} 


==> figures/hemisphere.tex <==
  \tdplotsetmaincoords{70}{105}
\pgfmathsetmacro{\rvec}{1.0}
  \begin{tikzpicture}[scale=1.7,line join=bevel,tdplot_main_coords,%
    fill opacity=0]
    \tdplotsetpolarplotrange{0}{180}{-90}{90}
    \tdplotsphericalsurfaceplot[black]{36}{36}%
    {1}{gray}{white}%
    {\draw[color=black,->] (0,0,0)
      -- (\rvec,0,0) node[below=0.5ex,left=-0.4ex]{$z$};}%
      {\draw[color=black,->] (0,0,0)
        -- (0,\rvec,0) node[right=-0.4ex]{$x$};}%
        {\draw[color=black,->] (0,0,0)
          -- (0,0,\rvec) node[above=-0.4ex]{$y$};}%
    \tdplotsetpolarplotrange{0}{180}{270}{360}
    \tdplotsphericalsurfaceplot[black]{36}{36}{1}{gray}{white}{}{}{}
   \end{tikzpicture}


==> figures/qual_other_real_data.tex <==
    \quad
    \makebox[0.10\textwidth]{\scriptsize Object} 
    \makebox[0.10\textwidth]{\scriptsize Est. Normal} 
    \qquad
    \makebox[0.10\textwidth]{\scriptsize Object} 
    \makebox[0.10\textwidth]{\scriptsize Est. Normal} 
    \\
    \raisebox{0.3\height}{\rotatebox{90}{\scriptsize (a) Apple}}
    \includegraphics[width=0.10\textwidth,height=0.11\textwidth]{images/Results/Gourd/I_0017.jpg}
    \includegraphics[width=0.10\textwidth,height=0.11\textwidth]{images/Results/Gourd/SCPS/apple_DiLiGenT_1}
    \hspace{0.3em}
    \raisebox{0.3\height}{\rotatebox{90}{\scriptsize (b) Gourd1}}
    \includegraphics[width=0.10\textwidth,height=0.11\textwidth]{images/Results/Gourd/I_0002.jpg}
    \includegraphics[width=0.10\textwidth,height=0.11\textwidth]{images/Results/Gourd/SCPS/gourd1_DiLiGenT_1}
    \\
    \raisebox{0.2\height}{\rotatebox{90}{\scriptsize (c) Helmet Front}}
    \includegraphics[width=0.1\textwidth,height=0.15\textwidth]{images/Results/LightStage/{20.0_helmet_front_left_0082}.jpg}
    \includegraphics[width=0.1\textwidth,height=0.15\textwidth]{images/Results/LightStage/SCPS/helmet_front_left_DiLiGenT_1.jpg}
    \hspace{0.3em}
    \raisebox{0.15\height}{\rotatebox{90}{\scriptsize (d) Fighting Knight}}
    \includegraphics[width=0.10\textwidth,height=0.15\textwidth]{images/Results/LightStage/{4.0_knight_standing_116}.jpg}
    \includegraphics[width=0.10\textwidth,height=0.15\textwidth]{images/Results/LightStage/SCPS/knight_standing_DiLiGenT_1.jpg}
    \\
    %\\
    %\includegraphics[width=0.10\textwidth]{images/Results/LightStage/{4.0_helmet_side_left_0192}.jpg}
    %\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/helmet_side_left_DiLiGenT_1.jpg}
    %\\
    %\includegraphics[width=0.1\textwidth]{images/Results/LightStage/{4.0_knight_fighting_057}.jpg}
    %\includegraphics[width=0.1\textwidth]{images/Results/LightStage/SCPS/knight_fighting_DiLiGenT_1.jpg}
    %\\
    %\includegraphics[width=0.10\textwidth]{images/Results/LightStage/{4.0_knight_kneeling_048}.jpg}
    %\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/knight_kneeling_DiLiGenT_1.jpg}
    %\\
    %\includegraphics[width=0.10\textwidth]{images/Results/LightStage/{4.0_plant_left_0021}.jpg}
    %\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/plant_left_DiLiGenT_1.jpg}
    %\\
    %\includegraphics[width=0.10\textwidth]{images/Results/Gourd/I_0027.jpg}
    %\includegraphics[width=0.10\textwidth]{images/Results/Gourd/SCPS/gourd2_DiLiGenT_1}


==> figures/res_qual_diligent.tex <==
 \makebox[0.115\textwidth]{\small Objects} 
 \makebox[0.115\textwidth]{\small GT Normal} 
 \makebox[0.23\textwidth]{\small UPS-FCN \cite{chen2018ps}}
 \makebox[0.23\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
 \makebox[0.23\textwidth]{\small SDPS-Net} 
 \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_ballPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_1_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_1_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_1_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_1_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_1_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_1_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_1_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_1_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_1_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_catPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_2_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_2_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_2_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_2_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_2_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_2_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_2_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_2_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_2_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_pot1PNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_3_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_3_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_3_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_3_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_3_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_3_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_3_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_3_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_3_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_bearPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_4_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_4_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_4_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_4_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_4_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_4_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_4_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_4_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_4_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_pot2PNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_5_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_5_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_5_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_5_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_5_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_5_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_5_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_5_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_5_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_buddhaPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_6_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_6_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_6_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_6_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_6_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_6_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_6_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_6_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_6_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_gobletPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_7_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_7_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_7_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_7_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_7_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_7_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_7_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_7_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_7_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_readingPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_8_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_8_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_8_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_8_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_8_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_8_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_8_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_8_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_8_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_cowPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_9_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_9_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_9_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_9_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_9_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_9_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_9_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_9_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_9_7}.jpg}
  \\
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{4.0_harvestPNG_001}.jpg}
            \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/GT/{1_10_4}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_10_3}.jpg}
  %\includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/PS-FCN_ECCV/{1_10_4}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_10_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/{1_10_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_10_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/End_to_end/{1_10_7}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_10_6}.jpg}
  \includegraphics[width=0.115\textwidth]{images/Results/DiLiGenT/SCPS/{1_10_7}.jpg}



==> figures/res_qual_light_diligent.tex <==
\begin{minipage}{0.45\textwidth}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/ballPNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/catPNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/pot1PNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/bearPNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/pot2PNG.jpg}
 \vspace{-1.8em}
 \\
 \makebox[0.19\textwidth]{\scriptsize ball}
 \makebox[0.19\textwidth]{\scriptsize cat}
 \makebox[0.19\textwidth]{\scriptsize pot1}
 \makebox[0.19\textwidth]{\scriptsize bear}
 \makebox[0.19\textwidth]{\scriptsize pot2}\\
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/buddhaPNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/gobletPNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/readingPNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/cowPNG.jpg}
 \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/harvestPNG.jpg}
 \vspace{-1.8em}
 \\
 \makebox[0.19\textwidth]{\scriptsize buddha}
 \makebox[0.19\textwidth]{\scriptsize goblet}
 \makebox[0.19\textwidth]{\scriptsize reading}
 \makebox[0.19\textwidth]{\scriptsize cow}
 \makebox[0.19\textwidth]{\scriptsize harvest}
\end{minipage}
\begin{minipage}{0.012\textwidth}
     \centering
     \makebox[0.16\textwidth]{\tiny $0\degree$}\\
     \vspace{0.2em}
     \includegraphics[width=0.5\linewidth]{images/Results/color_bar} \\
     \vspace{-0.4em}
     \makebox[0.16\textwidth]{\tiny$45\degree$}
\end{minipage}



==> figures/supple/qual_stage.tex <==
    \makebox[0.15\textwidth]{\small Objects} 
    \makebox[0.15\textwidth]{\small UPS-FCN \cite{chen2018ps}}
    \makebox[0.15\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
    \makebox[0.15\textwidth]{\small SDPS-Net} 
    \makebox[0.10\textwidth]{\small SDPS-Net Dir. Err.} 
    \\
    \raisebox{0.2\height}{\rotatebox{90}{\small (a) Helmet Side}}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/{4.0_helmet_side_left_0192}.png}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/helmet_side_left_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/End_to_end/helmet_side_left_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/SCPS/helmet_side_left_Normal_DiLiGenT}
    \raisebox{0.2\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/helmet_side_left}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\
    \raisebox{0.5\height}{\rotatebox{90}{\small (b) Helmet Front}}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/{4.0_helmet_front_left_0082}.png}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/helmet_front_left_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/End_to_end/helmet_front_left_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/SCPS/helmet_front_left_Normal_DiLiGenT}
    \raisebox{0.6\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/helmet_front_left}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-10em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\
    \raisebox{0.5\height}{\rotatebox{90}{\small (c) Fighting Knight}}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/{4.0_knight_fighting_057}.png}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/knight_fighting_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/End_to_end/knight_fighting_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/SCPS/knight_fighting_Normal_DiLiGenT}
    \raisebox{0.8\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/knight_fighting}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-12em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\
    \raisebox{0.0\height}{\rotatebox{90}{\footnotesize (d) Kneeling Knight}}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/{4.0_knight_kneeling_048}.png}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/knight_kneeling_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/End_to_end/knight_kneeling_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/SCPS/knight_kneeling_Normal_DiLiGenT}
    \raisebox{0.2\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/knight_kneeling}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\
    \raisebox{0.2\height}{\rotatebox{90}{\small (e) Standing Knight}}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/{4.0_knight_standing_116}.png}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/knight_standing_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/End_to_end/knight_standing_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/SCPS/knight_standing_Normal_DiLiGenT}
    \raisebox{0.6\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/knight_standing}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-10em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\
    \raisebox{0.4\height}{\rotatebox{90}{\small (d) Plant}}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/{2.0_plant_left_0021}}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/plant_left_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/End_to_end/plant_left_Normal_DiLiGenT}
    \includegraphics[width=0.148\textwidth]{images/Results/LightStage/SCPS/plant_left_Normal_DiLiGenT}
    \raisebox{0.0\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/plant_left}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\


==> figures/supple/qual_stage1.tex <==
    \makebox[0.21\textwidth]{\small Objects} 
    \makebox[0.21\textwidth]{\small UPS-FCN \cite{chen2018ps}}
    \makebox[0.21\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
    \makebox[0.21\textwidth]{\small SDPS-Net} 
    \makebox[0.10\textwidth]{\small SDPS-Net Dir. Err.} 
    \\
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/{4.0_helmet_side_left_helmet_side_left_0192}.png}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/helmet_side_left_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/End_to_end/helmet_side_left_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/SCPS/helmet_side_left_Normal_DiLiGenT}
    \raisebox{0.2\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/helmet_side_left}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \makebox{\small (a) {\sc Helmet Side}} \\
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/{4.0_helmet_front_left_helmet_front_left_0082}.png}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/helmet_front_left_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/End_to_end/helmet_front_left_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/SCPS/helmet_front_left_Normal_DiLiGenT}
    \raisebox{0.6\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/helmet_front_left}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-10em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \makebox{\small (b) {\sc Helmet Front}} \\
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/{2.0_plant_left_plant_left_0021}.png}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/plant_left_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/End_to_end/plant_left_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/SCPS/plant_left_Normal_DiLiGenT}
    \raisebox{0.0\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/plant_left}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \makebox{\small (c) {\sc Plant}} \\


==> figures/supple/qual_stage2.tex <==
    \makebox[0.21\textwidth]{\small Objects} 
    \makebox[0.21\textwidth]{\small UPS-FCN \cite{chen2018ps}}
    \makebox[0.21\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
    \makebox[0.21\textwidth]{\small SDPS-Net} 
    \makebox[0.10\textwidth]{\small SDPS-Net Dir. Err.} 
    \\
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/{4.0_knight_fighting_knight_fighting_057}.png}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/knight_fighting_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/End_to_end/knight_fighting_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/SCPS/knight_fighting_Normal_DiLiGenT}
    \raisebox{0.8\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/knight_fighting}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-12em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \makebox{\small (a) {\sc Fighting Knight}}
    \\
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/{4.0_knight_kneeling_knight_kneeling_048}.png}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/knight_kneeling_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/End_to_end/knight_kneeling_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/SCPS/knight_kneeling_Normal_DiLiGenT}
    \raisebox{0.2\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/knight_kneeling}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \makebox{\small (b) {\sc Kneeling Knight}}
    \\
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/{4.0_knight_standing_knight_standing_116}.png}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/UPS-FCN_ECCV/knight_standing_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/End_to_end/knight_standing_Normal_DiLiGenT}
    \includegraphics[width=0.21\textwidth]{images/Results/LightStage/SCPS/knight_standing_Normal_DiLiGenT}
    \raisebox{0.6\height}{\includegraphics[width=0.10\textwidth]{images/Results/LightStage/SCPS/knight_standing}}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-10em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \makebox{\small (c) {\sc Standing Knight}}


==> figures/supple/res_qual_diligent_compare.tex <==
\begin{minipage}{0.97\textwidth}\centering
 \makebox[0.15\textwidth]{\small GT / Object} 
 \makebox[0.15\textwidth]{\small SDPS-Net} 
 \makebox[0.15\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
 \makebox[0.15\textwidth]{\small UPS-FCN \cite{chen2018ps}}
 \makebox[0.15\textwidth]{\small PF14 \cite{papad14closed}} 
 \makebox[0.15\textwidth]{\small WT13 \cite{wu2013calib}} 
  \\
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/ballPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/ballPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/ballPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/ballPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/ballPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/ballPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_ballPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/ballPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/ballPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/ballPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/ballPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/ballPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (a) {\sc ball}} 
 \makebox[0.15\textwidth]{\small 2.77} 
 \makebox[0.15\textwidth]{\small 3.96} 
 \makebox[0.15\textwidth]{\small 6.62} 
 \makebox[0.15\textwidth]{\small 4.77} 
 \makebox[0.15\textwidth]{\small 4.39} 
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/catPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/catPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/catPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/catPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/catPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/catPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_catPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/catPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/catPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/catPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/catPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/catPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (b) {\sc cat}} 
 \makebox[0.15\textwidth]{\small 8.06} 
 \makebox[0.15\textwidth]{\small 12.16} 
 \makebox[0.15\textwidth]{\small 14.68} 
 \makebox[0.15\textwidth]{\small 9.54} 
 \makebox[0.15\textwidth]{\small 36.55} 
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/bearPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/bearPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/bearPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/bearPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/bearPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/bearPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_bearPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/bearPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/bearPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/bearPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/bearPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/bearPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (c) {\sc bear}} 
 \makebox[0.15\textwidth]{\small 6.89} 
 \makebox[0.15\textwidth]{\small 7.19} 
 \makebox[0.15\textwidth]{\small 11.23} 
 \makebox[0.15\textwidth]{\small 9.07} 
 \makebox[0.15\textwidth]{\small 6.42} 
\end{minipage}
    \begin{minipage}{0.02\textwidth} \centering
         \makebox[0.16\textwidth]{\small $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\small$90\degree$}\\
    \end{minipage}
    \\


==> figures/supple/res_qual_diligent_compare2.tex <==
\begin{minipage}{0.97\textwidth}\centering
 \makebox[0.15\textwidth]{\small GT / Object} 
 \makebox[0.15\textwidth]{\small SDPS-Net} 
 \makebox[0.15\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
 \makebox[0.15\textwidth]{\small UPS-FCN \cite{chen2018ps}}
 \makebox[0.15\textwidth]{\small PF14 \cite{papad14closed}} 
 \makebox[0.15\textwidth]{\small WT13 \cite{wu2013calib}} 
  \\
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/pot2PNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/pot2PNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/pot2PNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/pot2PNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot2PNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot2PNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_pot2PNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/pot2PNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/pot2PNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/pot2PNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot2PNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot2PNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (a) {\sc pot2}} 
 \makebox[0.15\textwidth]{\small 7.50} 
 \makebox[0.15\textwidth]{\small 11.11} 
 \makebox[0.15\textwidth]{\small 14.19} 
 \makebox[0.15\textwidth]{\small 15.90} 
 \makebox[0.15\textwidth]{\small 14.52} 
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/buddhaPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/buddhaPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/buddhaPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/buddhaPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/buddhaPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/buddhaPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_buddhaPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/buddhaPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/buddhaPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/buddhaPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/buddhaPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/buddhaPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (b) {\sc buddha}} 
 \makebox[0.15\textwidth]{\small 8.97} 
 \makebox[0.15\textwidth]{\small 13.06}
 \makebox[0.15\textwidth]{\small 15.87}
 \makebox[0.15\textwidth]{\small 14.92}
 \makebox[0.15\textwidth]{\small 13.19}
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/gobletPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/gobletPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/gobletPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/gobletPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/gobletPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/gobletPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_gobletPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/gobletPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/gobletPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/gobletPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/gobletPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/gobletPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (c) {\sc goblet}} 
 \makebox[0.15\textwidth]{\small 11.91} 
 \makebox[0.15\textwidth]{\small 18.07}
 \makebox[0.15\textwidth]{\small 20.72}
 \makebox[0.15\textwidth]{\small 29.93}
 \makebox[0.15\textwidth]{\small 20.57}
\end{minipage}
    \begin{minipage}{0.02\textwidth} \centering
         \makebox[0.16\textwidth]{\small $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\small$90\degree$}\\
    \end{minipage}
    \\


==> figures/supple/res_qual_diligent_compare3.tex <==
\begin{minipage}{0.97\textwidth}\centering
 \makebox[0.15\textwidth]{\small GT / Object} 
 \makebox[0.15\textwidth]{\small SDPS-Net} 
 \makebox[0.15\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
 \makebox[0.15\textwidth]{\small UPS-FCN \cite{chen2018ps}}
 \makebox[0.15\textwidth]{\small PF14 \cite{papad14closed}} 
 \makebox[0.15\textwidth]{\small WT13 \cite{wu2013calib}} 
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/pot1PNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/pot1PNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/pot1PNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/pot1PNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot1PNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot1PNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_pot1PNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/pot1PNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/pot1PNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/pot1PNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot1PNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/pot1PNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (a) {\sc pot1}} 
 \makebox[0.15\textwidth]{\small 8.14} 
 \makebox[0.15\textwidth]{\small 11.13} 
 \makebox[0.15\textwidth]{\small 13.98} 
 \makebox[0.15\textwidth]{\small 9.51} 
 \makebox[0.15\textwidth]{\small 9.39} 
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/readingPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/readingPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/readingPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/readingPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/readingPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/readingPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_readingPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/readingPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/readingPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/readingPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/readingPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/readingPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (b) {\sc reading}} 
 \makebox[0.15\textwidth]{\small 14.90}
 \makebox[0.15\textwidth]{\small 20.46}
 \makebox[0.15\textwidth]{\small 23.26}
 \makebox[0.15\textwidth]{\small 24.18}
 \makebox[0.15\textwidth]{\small 58.96}
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/cowPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/cowPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/cowPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/cowPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/cowPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/cowPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_cowPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/cowPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/cowPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/cowPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/cowPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/cowPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (c) {\sc cow}} 
 \makebox[0.15\textwidth]{\small 8.48} 
 \makebox[0.15\textwidth]{\small 11.84} 
 \makebox[0.15\textwidth]{\small 11.91}
 \makebox[0.15\textwidth]{\small 19.53}
 \makebox[0.15\textwidth]{\small 19.75}
  \\
  \vspace{1em}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/harvestPNGGT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/harvestPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/harvestPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/harvestPNGDiLiGenT_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/harvestPNGCVPR12Favaro_normal}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/harvestPNGCVPR13Wu_normal}
  \\
  \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/GT/{4.0_harvestPNG_001}.png}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/SCPS/harvestPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/End_to_end/harvestPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/UPS-FCN_ECCV/harvestPNGDiLiGenT_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/harvestPNGCVPR12Favaro_diff}
 \includegraphics[width=0.15\textwidth]{images/Results/DiLiGenT/compare/harvestPNGCVPR13Wu_diff}\\
 \makebox[0.15\textwidth]{\small (d) {\sc harvest}} 
 \makebox[0.15\textwidth]{\small 17.43}
 \makebox[0.15\textwidth]{\small 27.22}
 \makebox[0.15\textwidth]{\small 27.79}
 \makebox[0.15\textwidth]{\small 29.21}
 \makebox[0.15\textwidth]{\small 55.51}
\end{minipage}
    \begin{minipage}{0.02\textwidth} \centering
         \makebox[0.16\textwidth]{\small $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\small$90\degree$}\\
    \end{minipage}
    \\


==> figures/supple/res_qual_gourd.tex <==
    \makebox[0.19\textwidth]{\small Objects} 
    \makebox[0.19\textwidth]{\small UPS-FCN \cite{chen2018ps}}
    \makebox[0.19\textwidth]{\small UPS-FCN$_\text{deep+mask}$} 
    \makebox[0.19\textwidth]{\small SDPS-Net} 
    \makebox[0.15\textwidth]{\small SDPS-Net Dir. Err.} 
    \\
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/{2.0_apple_I_0003}.png}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/UPS-FCN_ECCV/apple_Normal_DiLiGenT}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/End_to_end/apple_Normal_DiLiGenT}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/SCPS/apple_Normal_DiLiGenT}
    \includegraphics[width=0.13\textwidth]{images/Results/Gourd/SCPS/apple}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \vspace{-0.24em}\makebox[\textwidth]{\small (a) Apple} 
    \\
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/{2.0_gourd1_I_0003}.png}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/UPS-FCN_ECCV/gourd1_Normal_DiLiGenT}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/End_to_end/gourd1_Normal_DiLiGenT}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/SCPS/gourd1_Normal_DiLiGenT}
    \includegraphics[width=0.13\textwidth]{images/Results/Gourd/SCPS/gourd1}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \vspace{-0.24em}\makebox[\textwidth]{\small (b) Gourd 1} 
    \\
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/{2.0_gourd2_I_0003}.png}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/UPS-FCN_ECCV/gourd2_Normal_DiLiGenT}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/End_to_end/gourd2_Normal_DiLiGenT}
    \includegraphics[width=0.19\textwidth]{images/Results/Gourd/SCPS/gourd2_Normal_DiLiGenT}
    \includegraphics[width=0.13\textwidth]{images/Results/Gourd/SCPS/gourd2}
    \begin{minipage}{0.012\textwidth} \centering
         \vspace{-6em} \makebox[0.16\textwidth]{\tiny $0\degree$}\\ \vspace{0.2em}
         \includegraphics[width=0.6\linewidth]{images/Results/color_bar} \\ \vspace{-0.4em}
         \makebox[0.16\textwidth]{\tiny$45\degree$}\\
    \end{minipage}
    \\ \vspace{-0.24em}\makebox[\textwidth]{\small (c) Gourd 2} 


==> tables/res_quant_light_diligent.tex <==
\resizebox{\textwidth}{!}{
            \huge
	         \begin{tabular}{c|*{10}{c}|c}
            \toprule
            & {\sc ball}         & {\sc cat}          & {\sc pot1}         & {\sc bear}         & {\sc pot2}         & {\sc buddha}        & {\sc goblet}         &{\sc reading}         & {\sc cow}            &{\sc harvest}        & Avg.\\
            \midrule
     Dir. & 3.27	 & 4.08	 & 5.44	 & 3.47	 & 2.87	 & 4.34	 & 10.36	 & 4.50	 & 4.52	 & 6.32	 & 4.92 \\
	 Int. & 0.039	 & 0.095	 & 0.058	 & 0.061	 & 0.048	 & 0.048	 & 0.067	 & 0.105	 & 0.073	 & 0.082	 & 0.068 \\
	             \bottomrule
        \end{tabular}
}

%\begin{minipage}{0.77\textwidth}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/ballPNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/catPNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/pot1PNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/bearPNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/pot2PNG.jpg}
% \vspace{-2.1em}
% \\
% \makebox[0.19\textwidth]{\tiny ball}
% \makebox[0.19\textwidth]{\tiny cat}
% \makebox[0.19\textwidth]{\tiny pot1}
% \makebox[0.19\textwidth]{\tiny bear}
% \makebox[0.19\textwidth]{\tiny pot2}\\
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/buddhaPNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/gobletPNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/readingPNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/cowPNG.jpg}
% \includegraphics[width=0.19\textwidth]{images/Results/DiLiGenT/SCPS/harvestPNG.jpg}
% \vspace{-2.1em}
% \\
% \makebox[0.19\textwidth]{\tiny buddha}
% \makebox[0.19\textwidth]{\tiny goblet}
% \makebox[0.19\textwidth]{\tiny reading}
% \makebox[0.19\textwidth]{\tiny cow}
% \makebox[0.19\textwidth]{\tiny harvest}
%\end{minipage}
%\begin{minipage}{0.032\textwidth}
%     \centering
%     \makebox[0.16\textwidth]{\tiny $0\degree$}\\
%     \vspace{0.2em}
%     \includegraphics[width=0.5\linewidth]{images/Results/color_bar} \\
%     \vspace{-0.4em}
%     \makebox[0.16\textwidth]{\tiny$45\degree$}
%\end{minipage}


==> tables/res_quant_light_gourd_stage.tex <==
\resizebox{0.48\textwidth}{!}{
    \Large
        \begin{tabular}{c|*{3}{c}c|*{6}{c}c}
            \toprule
            & \multicolumn{4}{c|}{\textbf{Gourd\&Apple Dataset}} & \multicolumn{7}{c}{\textbf{Light Stage Data Gallery}} \\
            & {\sc Apple} & {\sc Gourd1} &{\sc Gourd2} & Avg. & \makecell{{\sc Helmet} \\ {\sc Side}}& {\sc Plant} & \makecell{{\sc Fighting} \\ {\sc Knight}} & \makecell{{\sc Kneeling} \\ {\sc Knight}} & \makecell{{\sc Standing} \\ {\sc Knight}} & \makecell{{\sc Helmet}\\{\sc Front }} & Avg.\\
            \midrule
            Dir. & 9.31	 & 4.07	 & 7.11	 & 6.83  & 6.57	 & 16.06	 & 15.95	 & 19.84	 & 11.60	 & 11.62	 & 13.61 \\
            Int. & 0.106 & 0.048& 0.186	 & 0.113 & 0.212	 & 0.170	 & 0.214	 & 0.199	 & 0.286	 & 0.248	 & 0.221 \\ 
            \bottomrule
        \end{tabular}
}

	 
	 

